Auto-Configuring Entity Resolution Pipelines

The same real-world entity (e.g., a movie, a restaurant, a person) may be described in various ways on different datasets. Entity Resolution (ER) aims to find such different descriptions of the same entity, this way improving data quality and, therefore, data value. However, an ER pipeline typically involves several steps (e.g., blocking, similarity estimation, clustering), with each step requiring its own configurations and tuning. The choice of the best configuration, among a vast number of possible combinations, is a dataset-specific and labor-intensive task both for novice and expert users, while it often requires some ground truth knowledge of real matches. In this work, we examine ways of automatically configuring a state of-the-art end-to-end ER pipeline based on pre-trained language models under two settings: (i) When ground truth is available. In this case, sampling strategies that are typically used for hyperparameter optimization can significantly restrict the search of the configuration space. We experimentally compare their relative effectiveness and time efficiency, applying them to ER pipelines for the first time. (ii) When no ground truth is available. In this case, labelled data extracted from other datasets with available ground truth can be used to train a regression model that predicts the relative effectiveness of parameter configurations. Experimenting with 11 ER benchmark datasets, we evaluate the relative performance of existing techniques that address each problem, but have not been applied to ER before.

==> tables/all_f1s.tex <==
\begin{table}[ht!]
\caption{All results (to be removed).}
\label{tab:dl-results}
\begin{tabular}{|p{0.5cm}|l|p{1.2cm}|p{1.2cm}|p{1cm}|l|}
\hline
\textbf{Test set} & \textbf{Dataset} & \textbf{Regressor} & \textbf{Predicted F1} & \textbf{Best F1} & \textbf{Perfo} \\
\hline
% \midrule
D1 & optuna & RFG & 56.77 & 78.43 & 0.72 \\
D2 & gridsearch & NN & 85.40 & 85.85 & 0.99 \\
D3 & all &  AutoGB & 57.42 & 59.19 & 0.97 \\
D4 & all & NN & 98.51 & 98.60 & 1.00 \\
D5 & optuna & RFG & 76.96 & 78.92 & 0.98 \\
D6 & optuna & XGB & 51.81 & 60.42 & 0.86 \\
D7 & all & RFG & 64.24 & 67.76 & 0.95 \\
D8 & all & RFG & 40.78 & 49.53 & 0.82 \\
D9 & optuna &  AutoET & 94.39 & 94.92 & 0.99 \\
D10 & all & LR & 55.80 & 56.12 & 0.99 \\
\bottomrule
\end{tabular}
\end{table}     


==> tables/automl_f1s_with_data_features.tex <==
\begin{table*}[t]
%{\small
\begin{center}  
\caption{Performance of AutoML on Problem 2. GB stands for Gradient Boosting \cite{Friedman2001GreedyFA_GB}, KNN for K-Nearest Neighbor \cite{Fix1989DiscriminatoryA_KNN} RF for Random Forest \cite{Breiman2001RandomF_RF} and ET for Extra Trees \cite{Geurts2006ExtremelyRT_ET}. In all cases, the search/training time is 12 hours and is omitted for brevity.} 
\vspace{-10pt}
\label{tab:autosklearn-results}
%\begin{tabular}{|c|c|l|c|c|c|p{2cm}|p{1.0cm}|p{1.0cm}|c|c|c|c|}
\begin{tabular}{|c|c|l|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Dat.} & Inst. & \multicolumn{1}{c|}{Learned} & \multirow{2}{*}{F1} & 
%GB-F1 & F1-Ratio & 
%Optimization \& Training time (h) & 
Prediction & ETEER & \multirow{2}{*}{LM} & \multirow{2}{*}{k} & Clust & Thres \\
& gen. & \multicolumn{1}{c|}{ensemble} & & 
%GB-F1 & F1-Ratio & 
%Optimization \& Training time (h) & 
time (s) & time (s) &  &  & ering & hold \\
\hline
\hline
D1 & sampl. & 0.38ET + 0.36RF + 0.14GB + 0.1KNN + 0.02GB & 55.35 
%& 78.43 & 0.71 & 12 
& 240 & 5.84 & st5 & 1 & UMC & 0.265900 \\
D2 & sampl. & 0.82ET + 0.12GB + 0.04RF + 0.02KNN & 81.94 
%85.85 & 0.95 & 12 
& 179 & 0.18 & st5 & 1 & KC & 0.172200 \\
D3 & sampl. & 0.54ET + 0.16ET + 0.14RF + 0.12GB + 0.04KNN & 57.79 & %59.19 & 0.98 & 12 & 
218 & 2.98 & st5 & 32 & UMC & 0.05 \\
D4 & all & 0.96RF + 0.04GB & 98.45 & 
%98.60 & 1.00 & 12 & 
28 & 0.38 & st5 & 1 & CCC & 0.874200 \\
D5 & sampl. & 0.78ET + 0.1GB + 0.06RF + 0.06KNN & 71.97 & 
%78.92 & 0.91 & 12 & 
249 & 2.77 & smpnet & 1 & KC & 0.665900 \\
D6 & sampl. & 0.4ET + 0.18RF + 0.18GB + 0.12GB + 0.12KNN & 55.98 & %60.42 & 0.93 & 12 &
253 & 1.23 & sminilm & 1 & KC & 0.630700 \\
D7 & all & 0.9RF + 0.06GB + 0.04GB & 62.17 & 
%67.76 & 0.92 & 12 & 
68 & 2.05 & st5 & 1 & UMC & 0.75 \\
D8 & sampl. & 0.52ET + 0.2RF + 0.12KNN + 0.1GB + 0.06GB & 40.77 & %49.53 & 0.82 & 12 & 
230 & 20.66 & st5 & 91 & KC & 0.050100 \\
D9 & all & 0.94RF + 0.06GB & 94.39 & 
%94.92 & 0.99 & 12 & 
40 & 35.18 & st5 & 92 & KC & 0.70 \\
D10 & sampl. & 0.78ET + 0.12GB + 0.1ET & 36.31 
%& 56.12 & 0.65 & 12 
& 68 & 13.65 & smpnet & 1 & KC & 0.05 \\
\hline
\end{tabular}
\end{center}  
%}
\vspace{-10pt}
\end{table*}

%Test set & Trials training set & Regressor ensembled & F1 & GB-F1 & F1-Ratio & Optimization \& Training time (h) & Prediction time (s) & ETEER Runtime (s) & LM & k & Clustering & Threshold \\
%\midrule
%D1 & sampl. & 0.38ET + 0.36RF + 0.14GB + 0.1KNN + 0.02GB & 55.35 & 78.43 & 0.71 & 12 & 240 & 5.84 & st5 & 1 & UMC & 0.265900 \\
%D2 & sampl. & 0.82ET + 0.12GB + 0.04RF + 0.02KNN & 81.94 & 85.85 & 0.95 & 12 & 179 & 0.18 & st5 & 1 & KC & 0.172200 \\
%D3 & sampl. & 0.54ET + 0.16ET + 0.14RF + 0.12GB + 0.04KNN & 57.79 & 59.19 & 0.98 & 12 & 218 & 2.98 & st5 & 32 & UMC & 0.05 \\
%D4 & all & 0.96RF + 0.04GB & 98.45 & 98.60 & 1.00 & 12 & 28 & 0.38 & st5 & 1 & CCC & 0.874200 \\
%D5 & sampl. & 0.78ET + 0.1GB + 0.06RF + 0.06KNN & 71.97 & 78.92 & 0.91 & 12 & 249 & 2.77 & smpnet & 1 & KC & 0.665900 \\
%D6 & sampl. & 0.4ET + 0.18RF + 0.18GB + 0.12GB + 0.12KNN & 55.98 & 60.42 & 0.93 & 12 & 253 & 1.23 & sminilm & 1 & KC & 0.630700 \\
%D7 & all & 0.9RF + 0.06GB + 0.04GB & 62.17 & 67.76 & 0.92 & 12 & 68 & 2.05 & st5 & 1 & UMC & 0.75 \\
%D8 & sampl. & 0.52ET + 0.2RF + 0.12KNN + 0.1GB + 0.06GB & 40.77 & 49.53 & 0.82 & 12 & 230 & 20.66 & st5 & 91 & KC & 0.050100 \\
%D9 & all & 0.94RF + 0.06GB & 94.39 & 94.92 & 0.99 & 12 & 40 & 35.18 & st5 & 92 & KC & 0.70 \\
%D10 & sampl. & 0.78ET + 0.12GB + 0.1ET & 36.31 & 56.12 & 0.65 & 12 & 68 & 13.65 & smpnet & 1 & KC & 0.05 \\

==> tables/automl_f1s_without_data_features.tex <==
\begin{table*}[ht!]
{\footnotesize
\begin{center}  
\caption{Learning procedure 1 (AutoML) results. \textbf{WITHOUT Data Features.} GB:Gradient Boosting, RF:Random Forest, ET:Extra Trees, KNN:K-Nearest Neighbor, AD:AdaBoost, ARD:ARD Regression } 
\label{tab:autosklearn-results}
\begin{tabular}{|c|c|p{2.5cm}|c|c|c|p{2cm}|p{1.0cm}|p{1.0cm}|c|c|c|c|}
\toprule
Test set & Trials training set & Regressor ensembled & F1 & GB-F1 & F1-Ratio & Optimization \& Training time (h) & Prediction time (s) & ETEER Runtime (h) & LM & k & Clustering & Threshold \\
\midrule
D1 & all & 0.54GB + 0.36RF + 0.1GB & 57.14 & 78.43 & 0.73 & 12 & 62 & 12.02 & st5 & 1 & KMAC & 0.7790 \\
D2 & optuna & 0.92ET + 0.02ET + 0.02GB + 0.02KNN + 0.02AD & 78.63 & 85.85 & 0.92 & 12 & 61 & 12.02 & st5 & 12 & KMAC & 0.111700 \\
D3 & all & 0.62GB + 0.36RF + 0.02GB & 57.42 & 59.19 & 0.97 & 12 & 56 & 12.01 & st5 & 100 & KMAC & 0.3017 \\
D4 & all & 0.66GB + 0.32RF + 0.02GB & 98.18 & 98.60 & 1.00 & 12 & 69 & 12.02 & st5 & 21 & KMAC & 0.3019 \\
D5 & gridsearch & 0.72RF + 0.14AD + 0.12ARD + 0.02AD & 72.87 & 78.92 & 0.92 & 12 & 17 & 12.00 & st5 & 81 & KMAC & 0.70 \\
D6 & optuna & 0.86ET + 0.04ET + 0.04GB + 0.04KNN + 0.02ARD & 51.16 & 60.42 & 0.85 & 12 & 56 & 12.02 & sminilm & 1 & UMC & 0.20 \\
D7 & all & 0.58GB + 0.36RF + 0.06GB & 65.47 & 67.76 & 0.97 & 12 & 68 & 12.02 & sminilm & 1 & UMC & 0.6694 \\
D8 & optuna & 0.9ET + 0.02GB + 0.02AD + 0.02KNN + 0.02RF + 0.02RF & 47.05 & 49.53 & 0.95 & 12 & 62 & 12.02 & st5 & 1 & UMC & 0.8960 \\
D9 & optuna & 0.86ET + 0.1RF + 0.04GB & 94.39 & 94.92 & 0.99 & 12 & 25 & 12.02 & st5 & 21 & KMAC & 0.3019 \\
D10 & all & 0.6GB + 0.36RF + 0.04GB & 55.40 & 56.12 & 0.99 & 12 & 50 & 12.01 & st5 & 1 & KMAC & 0.1932 \\
\bottomrule
\end{tabular}
\end{center}  
}
\end{table*}

==> tables/dataset_features.tex <==
\begin{table}[t]
{\footnotesize
\begin{center}  
\label{tab:featureSet}
\begin{tabular}{|p{2cm}|p{5cm}|}\hline
\textbf{Dataset Feature} & \textbf{Definition} \\
\hline
Number of entities & The total number of entities in the dataset \\ \hline
Number of attributes & The total number of attributes for the entities \\ \hline
Number of distinct values & The total number of distinct values across all attributes \\ \hline
Number of name-value pairs & The total number of name-value pairs in the dataset \\ \hline
Mean name-value pairs per entity & The average number of name-value pairs per entity \\ \hline
Mean name-value pairs per attribute & The average number of name-value pairs per attribute \\ \hline
Number of missing name-value pairs & The total number of missing name-value pairs in the dataset \\ \hline
Mean distinct values per attribute & The average number of distinct values per attribute \\ \hline
Mean total attribute value length per entity & The average total length of attribute values per entity \\ \hline
Mean attribute value tokens per entity & The average number of tokens in attribute values per entity \\ \hline
Mean distinct values per entity & The average number of distinct values per entity \\ \hline
Max values per entity & The maximum number of values for any single entity \\ \hline
\end{tabular}
\caption{The list of dataset features.}
\end{center}  
}
\end{table}

==> tables/default_conf_performance.tex <==
\begin{table*}[ht!]
\centering
\caption{Default F1s for pipeline (st5, 10, UniqueMappingClustering, 0.5).}
\label{tab:global-bestf1s}
\begin{tabular}{|c|c|c|}
\toprule
Dataset & F1 & Runtime (s)\\
\midrule
D1 & 47.44 & 1.90 \\
D2 & 85.85 & 3.28 \\
D3 & 57.35 & 1.49 \\
D4 & 97.56 & 4.45 \\
D5 & 57.74 & 5.05 \\
D6 & 30.39 & 1.81 \\
D7 & 35.68 & 2.21 \\
D8 & 35.82 & 4.46 \\
D9 & 92.04 & 13.11 \\
D10 & 53.63 & 27.96 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/ditto.tex <==
\begin{table}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{1.4pt}
\caption{Performance of DITTO over the datasets.}
\vspace{-10pt}
\label{tab:zeroer-results}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\cline{2-11}
\multicolumn{1}{c|}{} & D1 & D2 & D3 & D4 & D5 & D6 & D7 & D8 & D9 & D10 \\
\hline
\hline
F1 & 74.29 & 19.01 & 64.06 & 98.83 & 88.44 & 2.43 & 2.60 & 58.49 & 0.76 & 10.49 \\
RT & 1138 & 566 & 1979 & 1097 & 3821 & 755 & 4993 & 9543 & 25722 & 8290 \\
\hline
\end{tabular}
\vspace{-8pt}
\end{table}

==> tables/dl_f1s.tex <==
\begin{table}[ht!]
\caption{DL results (to be removed).}
\label{tab:dl-results}
\begin{tabular}{|p{0.5cm}|l|p{1.2cm}|p{1.2cm}|p{1cm}|l|}
\hline
\textbf{Test set} & \textbf{Dataset} & \textbf{Regressor} & \textbf{Predicted F1} & \textbf{Best F1} & \textbf{Performance} \\
\hline
% \midrule
D1 & optuna & NN & 54.83 & 77.0833 & 0.7113 \\
D2 & optuna & NN & 85.78 & 85.8486 & 0.9992 \\
D3 & optuna & NN & 57.78 & 59.0871 & 0.9779 \\
D4 & optuna & NN & 98.38 & 98.5122 & 0.9986 \\
D5 & optuna & NN & 70.53 & 78.2517 & 0.9014 \\
D6 & all & NN & 38.99 & 60.2534 & 0.6471 \\
D7 & optuna & NN & 63.68 & 67.7308 & 0.9402 \\
D8 & all & NN & 40.12 & 48.5417 & 0.8265 \\
D9 & all & NN & 92.33 & 94.9211 & 0.9727 \\
D10 & gridsearch & NN & 56.11 & 56.117 & 0.9999 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/dl_searchspace.tex <==
\begin{table}[t]
\centering
\caption{Parameters Tested for the Neural Network}
\label{tab:nn_params}
\begin{tabular}{|l|l|}
\hline
\textbf{Parameter} & \textbf{Search Space}      \\ \hline
hidden\_dim        & int(16, 128)               \\ \hline
lr                 & loguniform(1e-5, 1e-2)     \\ \hline
num\_epochs        & int(2, 50)                 \\ \hline
\end{tabular}
\end{table}

==> tables/lr_with_data_features_performance.tex <==
\begin{table}[t]
{\small
\begin{center}  
\setlength{\tabcolsep}{2pt}
\caption{Performance of Random Forest on Problem 2.} 
\vspace{-10pt}
\label{tab:lr-with-data-features}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Dat.} & Insta. & \multirow{2}{*}{F1} & Train.  & Predic.  & ETEER  & \multirow{2}{*}{LM} & \multirow{2}{*}{k} & Clust & Thre \\
 & gen. & & time (s) & time (s) &  time (s) &  &  & ering & shold \\
\hline
\hline
D1 & all & 56.77 & 0.72 & 0.02 & 2.88 & st5 & 1 & UMC & 0.73 \\
D2 & grid. & 78.46 & 0.91 & 0.01 & 5.10 & st5 & 16 & KC & 0.10 \\
D3 & grid. & 56.86 & 0.96 & 0.01 & 0.55 & st5 & 2 & KC & 0.60 \\
D4 & grid. & 98.24 & 1.00 & 0.01 & 1.70 & st5 & 2 & KC & 0.20 \\
D5 & opt. & 76.75 & 0.97 & $\ll$0.01 & 1.91 & sminilm & 1 & UMC & 0.65 \\
D6 & opt. & 53.31 & 0.88 & 0.01 & 1.34 & sminilm & 1 & KC & 0.65 \\
D7 & grid. & 62.12 & 0.92 & 0.01 & 1.58 & sminilm & 1 & KC & 0.60 \\
D8 & all & 40.78 & 0.82 & 0.01 & 28.79 & st5 & 100 & KC & 0.22 \\
D9 & all & 94.37 & 0.99 & 0.01 & 60.20 & st5 & 100 & KC & 0.38 \\
D10 & grid. & 54.91 & 0.98 & 0.01 & 37.55 & st5 & 27 & KC & 0.50 \\
\hline
\end{tabular}
\end{center}  
}
\vspace{-10pt}
\end{table}
%\toprule
% D1 & all & RFR & 56.77 & 78.43 & 0.72 & 130.55 & 1.60 & 2.88 & st5 & 1 & UMC & 0.733563 \\
% D2 & gridsearch & RFR & 78.46 & 85.85 & 0.91 & 10.10 & 0.18 & 5.10 & st5 & 16 & KC & 0.10 \\
% D3 & gridsearch & RFR & 56.86 & 59.19 & 0.96 & 10.22 & 0.18 & 0.55 & st5 & 2 & KC & 0.60 \\
% D4 & gridsearch & RFR & 98.24 & 98.60 & 1.00 & 65.26 & 1.00 & 1.70 & st5 & 2 & KC & 0.20 \\
% D5 & optuna & RFR & 76.75 & 78.92 & 0.97 & 5.25 & 0.05 & 1.91 & sminilm & 1 & UMC & 0.651879 \\
% D6 & optuna & RFR & 53.31 & 60.42 & 0.88 & 20.30 & 0.19 & 1.34 & sminilm & 1 & KC & 0.647542 \\
% D7 & gridsearch & RFR & 62.12 & 67.76 & 0.92 & 38.81 & 0.47 & 1.58 & sminilm & 1 & KC & 0.60 \\
% D8 & all & RFR & 40.78 & 49.53 & 0.82 & 27.48 & 0.29 & 28.79 & st5 & 100 & KC & 0.219945 \\
% D9 & all & RFR & 94.37 & 94.92 & 0.99 & 67.96 & 0.80 & 60.20 & st5 & 100 & KC & 0.375625 \\
% D10 & gridsearch & RFR & 54.91 & 56.12 & 0.98 & 48.67 & 0.67 & 37.55 & st5 & 27 & KC & 0.50 \\
%Test set & Trials training set & Regressor & F1 & GB-F1 & F1-Ratio & Training time (s) & Prediction time (s) & ETEER runtime (s) & LM & k & Clustering & Threshold \\
%\midrule
%D1 & all & LR & 55.35 & 78.43 & 0.71 & 0.33 & 0.01 & 0.24 & st5 & 1 & KC & 0.05 \\
%D2 & all & LR & 81.94 & 85.85 & 0.95 & 0.24 & $\ll$0.01 & 0.20 & st5 & 1 & KC & 0.05 \\
%D3 & all & LR & 55.98 & 59.19 & 0.95 & 0.33 & $\ll$0.01 & 0.48 & st5 & 1 & KC & 0.05 \\
%D4 & all & LR & 98.38 & 98.60 & 1.00 & 0.21 & $\ll$0.01 & 0.83 & st5 & 1 & KC & 0.05 \\
%D5 & all & LR & 69.39 & 78.92 & 0.88 & 0.21 & $\ll$0.01 & 0.79 & st5 & 1 & KC & 0.05 \\
%D6 & optuna & LR & 46.65 & 60.42 & 0.77 & 0.06 & $\ll$0.01 & 10.24 & st5 & 100 & KC & 0.05 \\
%D7 & all & LR & 48.48 & 67.76 & 0.72 & 0.21 & $\ll$0.01 & 1.62 & st5 & 1 & KC & 0.05 \\
%D8 & all & LR & 38.09 & 49.53 & 0.77 & 0.21 & $\ll$0.01 & 1.63 & st5 & 1 & KC & 0.05 \\
%D9 & all & LR & 92.85 & 94.92 & 0.98 & 0.21 & $\ll$0.01 & 4.23 & st5 & 1 & KC & 0.05 \\
%D10 & gridsearch & LR & 55.40 & 56.12 & 0.99 & 0.22 & 0.01 & 12.54 & st5 & 1 & KC & 0.05 \\
%\bottomrule

==> tables/lr_without_data_features.tex <==
\begin{table*}[ht!]
{\footnotesize
\begin{center}  
\caption{Learning procedure 2 (Linear Regression) results. \textbf{WITHOUT Data Features.}} 
\label{tab:lr-without-data-features}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
Test set & Trials training set & Regressor & F1 & GB-F1 & F1-Ratio & Training time (s) & Prediction time (s) & ETEER Runtime (s) & LM & k & Clustering & Threshold \\
\midrule
D1 & optuna & LR & 55.35 & 78.43 & 0.71 & 0.02 & 0.00 & 0.02 & st5 & 1 & KMAC & 0.05 \\
D2 & optuna & LR & 81.94 & 85.85 & 0.95 & 0.02 & 0.00 & 0.02 & st5 & 1 & KMAC & 0.05 \\
D3 & optuna & LR & 55.98 & 59.19 & 0.95 & 0.02 & 0.00 & 0.02 & st5 & 1 & KMAC & 0.05 \\
D4 & all & LR & 98.38 & 98.60 & 1.00 & 0.08 & 0.00 & 0.078 & st5 & 1 & KMAC & 0.05 \\
D5 & optuna & LR & 69.39 & 78.92 & 0.88 & 0.02 & 0.00 & 0.02 & st5 & 1 & KMAC & 0.05 \\
D6 & optuna & LR & 43.85 & 60.42 & 0.73 & 0.02 & 0.00 & 0.022 & st5 & 1 & KMAC & 0.05 \\
D7 & optuna & LR & 48.48 & 67.76 & 0.72 & 0.02 & 0.00 & 0.022 & st5 & 1 & KMAC & 0.05 \\
D8 & optuna & LR & 38.09 & 49.53 & 0.77 & 0.02 & 0.00 & 0.022 & st5 & 1 & KMAC & 0.05 \\
D9 & optuna & LR & 92.85 & 94.92 & 0.98 & 0.02 & 0.00 & 0.022 & st5 & 1 & KMAC & 0.05 \\
D10 & gridsearch & LR & 55.40 & 56.12 & 0.99 & 0.04 & 0.00 & 0.04 & st5 & 1 & KMAC & 0.05 \\
\bottomrule
\end{tabular}
\end{center}  
}
\end{table*}

==> tables/sklearn_and_nn_f1s.tex <==
\begin{table}[t]
{\footnotesize
\begin{center}  
\caption{Learning Procedure 2 results (Individual regressors).}
\label{tab:sklearn-nn-results}
\begin{tabular}{|p{0.5cm}|l|p{1.2cm}|p{1.2cm}|p{1cm}|l|}
\hline
\textbf{Test set} & \textbf{Trials} & \textbf{Regressor} & \textbf{Predicted F1} & \textbf{Best F1} & \textbf{Performance} \\
\hline
D1 & optuna & RFR & 56.77 & 78.43 & 0.72 \\
D2 & gridsearch & NN & 85.40 & 85.85 & 0.99 \\
D3 & gridsearch & XGB & 56.88 & 59.19 & 0.96 \\
D4 & all & NN & 98.51 & 98.60 & 1.00 \\
+D5 & optuna & RFR & 76.96 & 78.92 & 0.98 \\
D6 & optuna & XGB & 51.81 & 60.42 & 0.86 \\
D7 & all & RFR & 64.24 & 67.76 & 0.95 \\
D8 & all & RFR & 40.78 & 49.53 & 0.82 \\
D9 & all & RFR & 94.37 & 94.92 & 0.99 \\
D10 & all & LR & 55.80 & 56.12 & 0.99 \\
\bottomrule
\end{tabular}
\end{center}  
}
\end{table}

==> tables/sklearn_nn_searchspace.tex <==
\begin{table}[ht]
\centering
\caption{Parameters Tested for RF Regression Method.}
\label{tab:regressor_params}
\begin{tabular}{|p{1.5cm}|l|l|}
\hline
\textbf{Regressor}          & \textbf{Parameter}        & \textbf{Search Space}                           \\ \hline
% \multirow{1}{*}{Lasso}      & alpha                     & \text{LogUniform}($10^{-4}$, $10^1$)                           \\ \hline
% \multirow{1}{*}{Ridge}      & alpha                     & \text{LogUniform}($10^{-4}$, $10^1$)                           \\ \hline
% \multirow{1}{*}{LR} & -                 & -                                               \\ \hline
% \multirow{8}{*}{XGBR} & n\_estimators    & $\{100,...,1000\} \subseteq \mathbb{Z}$                                   \\ \cline{2-3}
%                             & max\_depth                 & $\{3,...,10\} \subseteq \mathbb{Z}$                                      \\ \cline{2-3}
%                             & learning\_rate             & \text{LogUniform}($10^{-3}$, $10^{-1}$)                          \\ \cline{2-3}
%                             & subsample                 & \text{Uniform}($0.5$, $1.0$)                                                \\ \cline{2-3}
%                             & colsample\_bytree          & \text{Uniform}($0.5$, $1.0$)                               \\ \cline{2-3}
%                             & gamma                     & $\{0,...,5\} \subseteq \mathbb{Z}$                                        \\ \cline{2-3}
%                             & reg\_alpha                 & \text{LogUniform}($10^{-2}$, $10^{2}$)                              \\ \cline{2-3}
%                             & reg\_lambda                & \text{LogUniform}($10^{-2}$, $10^{2}$)                              \\ \hline
\multirow{5}{*}{RFR} & n\_estimators & $\{100, ..., 1000\} \subseteq \mathbb{Z}$                                  \\ \cline{2-3}
                            & max\_depth                 &  $\{3,...,10\} \subseteq \mathbb{Z}$                                      \\ \cline{2-3}
                            & min\_samples\_split         &  $\{2,...,20\} \subseteq \mathbb{Z}$                                      \\ \cline{2-3}
                            & min\_samples\_leaf          &  $\{1,...,20\} \subseteq \mathbb{Z}$                                      \\ \cline{2-3}
                            & max\_features              & $\{ sqrt, log2\}$                            \\ \hline
% \multirow{3}{*}{NN}         & hidden\_dim                &  $\{16,...,128\} \subseteq \mathbb{Z}$                                    \\ \cline{2-3}
%                             & lr                         & \text{LogUniform}($10^{-5}, 10^{-2}$)                          \\ \cline{2-3}
%                             & num\_epochs                &  $\{2,...,50\} \subseteq \mathbb{Z}$                                      \\ \hline
\end{tabular}
\end{table}

